Blowup of Jang's equation at outermost marginally trapped surfaces

The aim of this paper is to collect some facts about the blowup of Jang's equation. First, we discuss how to construct solutions that blow up at an outermost MOTS. Second, we exclude the possibility that there are extra blowup surfaces in data sets with non-positive mean curvature. Then we investigate the rate of convergence of the blowup to a cylinder near a strictly stable MOTS and show exponential convergence near a strictly stable MOTS.

==> boundary.tex <==
\section{A boundary term}
In \cite{Yau:2001} Yau used control of a certain boundary term in an
argument for an existence result for trapped surfaces. This term
proved very useful and allowed the exploitation of a boundary effect
to conclude existence. Here, we wish to examine the same boundary term
in the limit as $f\to\infty$ on the cylindrical end of $N=\graph f$,
where $f$ is the function constructed in theorem~\ref{thm:blowup} for
a data set $(M,g,K)$ as described in this theorem. Throughout this
section we assume that the boundary component we are working with is
strictly stable, so that we have the asymptotics from
theorem~\ref{thm:exponential}.

To introduce the term we are interested in, we first review some
formulas from \cite{Schoen-Yau:1981} and \cite{Jang:1978}. In the
discussion of this section we let $(M,g,K)$ and $f$ be as in
theorem~\ref{thm:blowup}. In the sequel, we denote by $\bar \nu$ the
downward normal to $N$ in $\bar M$. As before, $\pi$ denotes the
orthogonal projection onto $TM$. Furthermore, $\bar K^N$ denotes the
restriction of $\bar K$ to the tangent space of $N$ and $\bar A$ the
second fundamental form of $N$ in $\bar M$. Let $\alpha^2= 1 + |\nabla
f|^2$, where the gradient and its norm are computed on $M$. Denote
$v:= \alpha^{-1}$ and consider the 1-form $\xi$ tangential to $N$
which is given by
\begin{equation}
  \label{eq:11}
  \xi = \nabN \log v + \bar K(\bar\nu, \cdot)^T
\end{equation}
where $\bar K(\bar\nu, \cdot)^T$ denotes the projection of the 1-form
$\bar K(\bar\nu,\cdot)$ to $N$ and $\nabN$ denotes the tangential
gradient on $N$. Here, and in the sequel, we will consider all
functions on $M$ also as functions on $N$ by extending them constantly
along the vertical direction and restricting them to $N$. An analogous
construction works vice-versa.

If $f$ is a solution of Jang's equation we can calculate the scalar
curvature $\ScalN$ of $N = \graph f$
(cf.~\cite[(2.25)]{Schoen-Yau:1981} and \cite[(18)]{Jang:1978}):
\begin{equation}
  \label{eq:13}
  \half \ScalN = |\xi|^2 + \div\xi + \tfrac{1}{2} |\bar A - \bar K^N|^2 + \mu - J(\pi\bar\nu).
\end{equation}
Here
\begin{align*}
  \mu
  &=
  \half \big(\Scal M - |K|^2 + (\tr K)^2 \big)
  \\
  J
  &=
  \div K - \nabla \tr K.
\end{align*}
Using the dominant energy condition, that is $\mu \geq |J|$,
equation~\eqref{eq:13} implies the inequality
\begin{equation}
  \label{eq:8}
  \half \ScalN \geq |\xi|^2 + \div\xi.
\end{equation}
In a crucial step in their argument, Schoen and Yau
\cite{Schoen-Yau:1981} use \eqref{eq:8} to conclude that $N$ is of
non-negative Yamabe type. To do this, they multiply~\eqref{eq:8} by
$\eta^2$, where $\eta$ is a smooth, compactly supported test
function, and integrate:
\begin{equation}
  \label{eq:12}
  \begin{split}
    0
    &\leq
    \int_N \eta^2 (\half \ScalN  - |\xi|^2 -\div \xi) \dV
    \\
    &=
    \int_N  \eta^2
    (\half \ScalN  - |\xi|^2) + 2\eta \la \nabla \eta, \xi\ra
    \dV
    \\
    &\leq
    \int_N |\nabla\eta|^2 + \half\eta^2\ScalN\, \dV.
  \end{split}
\end{equation}
In a variant, we can now drop the assumption that $\eta$ vanishes on
the cylindrical end, and instead of $N$ we can consider the manifold
$N_z$ which is given by
\begin{equation*}
  N_z := \big\{ (x,f(x)) \in N : f(x) < z\big\}.
\end{equation*}
For large enough $z$ the manifold $N_z$ has the smooth boundary $S_z$
given by
\begin{equation*}
  \bar S_z := \big \{ (x,f(x)) \in N : f(x) = z\big\}.
\end{equation*}
Note here that the blow up near $\del^- M$ implies that for
$z\to\infty$ the surfaces $\bar S_z$ are in fact smooth submanifolds
of $N$. Denote by $S_z$ the projection of $\bar S_z$ to $M$, that is 
\begin{equation*}
  S_z := \big \{ x \in M : f(x) = z\big\}.
\end{equation*}
By theorem~\ref{thm:sideways}, these surfaces converge in the
$C^2$-norm to $\del^- M$, and the convergence is unidirectional in the
sense that the surface $S_z$ lies in the region bounded by $\del^- M$
and $S_{z'}$, provided $z>z'$.

If we now integrate over $N_z$ and do the partial integration as
in~\eqref{eq:12}, we are left with a boundary term
\begin{equation*}
     0
     \leq
     \int_{N_z} |\nabla\eta|^2 + \half \eta^2\ScalN\, \dV
     + \int_{S_z} \eta^2 \la \xi, \bar n\ra \dmu,
\end{equation*}
where $\bar n$ is the normal to $\bar S_z$ tangential to $N$ and
pointing downwards along the blowup cylinder.

As an interesting side note, in his original paper Jang
\cite{Jang:1978} not only introduced equation~\eqref{eq:1}, but also
a flow he used to study the positive energy (at that time)
conjecture. This flow is a modified version of inverse mean curvature
flow. In short, it is used to flow surfaces $\Sigma$ in $N$ along
their normal according to the equation
\begin{equation*}
  \dd{x}{t} = \frac{1}{H + \la\xi,\nu\ra}\nu
\end{equation*}
where $x$ is the position of the surface, $\nu$ its normal in $N$ and
$\xi$ as above. So if one would want to start the flow with say, a
surface $S_z$ very close to $\del M$, which in $N$ has mean curvature
close to zero, it it interesting whether the term $\la\xi,\nu\ra$ has
a sign, to determine if the flow initially moves outward or inward.

We will now examine the term $\la\xi,\bar n\ra$ on $S_z$, and in
particular try to identify its sign in the limit $z\to\infty$. To this
end, we introduce some notation. Let
\begin{equation*}
  V = \pi \bar \nu = \frac{\nabla f}{\alpha}.
\end{equation*}
As $\bar \nu$ is the normal vector of $N$ and $\del_z$, the vertical
direction, is parallel, we find
\begin{equation*}
  \bar H = \divN \bar \nu = \divN \pi\bar\nu = \divM V.
\end{equation*}
On the other hand
\begin{equation*}
  \divM V
  =
  \alpha^{-1}\big(
  \Delta f - \alpha^{-2}\nabla^2f(\nabla f,\nabla f)
  \big)  
\end{equation*}
Here $\nabla, \Delta$ and $\nabla^2$ denote the gradient, Laplacian
and Hessian with respect to $(M,g)$. Let $n$ denote the outward
pointing normal to $S_z$, then
\begin{equation*}
  n = - \frac{\nabla f}{|\nabla f|}.
\end{equation*}
The mean curvature of $S_z$ is given by
\begin{equation*}
  H
  =
  \div n
  =
  - |\nabla f|^{-1} \big(
  \Delta f - |\nabla f|^{-2}\nabla^2(\nabla f, \nabla f)
  \big).
\end{equation*}
Compute furthermore that
\begin{equation*}
  \nabla |V|
  =
  - \alpha^{-3}\nabla^2 f (n, \cdot),
\end{equation*}
so that we can express $\bar H$ in terms of $H$ as follows
\begin{equation*}
  \bar H = -|V| H - \nabla_n |V|.
\end{equation*}
Since
\begin{equation*}
  \bar P  = \tr K - K(V,V),
\end{equation*}
we thus infer that Jang's equation implies
\begin{equation*}
  -|V| H - \nabla_n |V| - \tr K + K(V,V) = 0.
\end{equation*}
We express $H = \theta^+ - P$ and $\tr K = P + K(n,n)$, where
$\theta^+$, $P$ and $K(n,n)$ are computed on $S_z$, and to infer
\begin{equation}
  \label{eq:14}
  \nabla_n |V| + |V|\theta^+ + (1- |V|) P + (1-|V|^2) K(n,n) = 0.
\end{equation}

Recall, that theorem~\ref{thm:sideways} implies the following
properties of $S_z$:
\begin{enumerate}
\item $S_z \to \del M$ in the $C^2$-norm as $z\to\infty$, in
  particular $\theta^+[S_z]\to 0$ uniformly, and 
\item $|\nabla f|\to \infty$ uniformly on $S_z$, in particular
  $|V|\to 1$ uniformly on $S_z$ as $z\to\infty$.
\end{enumerate}
As $P$ and $K(n,n)$ are bounded, equation~\eqref{eq:14} implies the
following.
\begin{proposition}
  \label{thm:phi_der}
  In the notation introduced above, 
  \begin{equation*}
    \nabla_n |V| \to 0
  \end{equation*}
  uniformly on $S_z$ as $z\to\infty$.
\end{proposition}
\begin{remark}
  If $\bar A$ denotes the second fundamental form of $N$, then we can
  calculate that $\nabla_n|V|(x) = \bar A_{(x,f(x))}(\bar n,\bar n)$,
  so the above result simply says that $N$ becomes flat in the $\bar
  n$ direction, which is clear in view of the fact that $N$ becomes
  cylindrical.
\end{remark}
Let us now go back to the boundary term $\la \xi,\bar n\ra$. We first
want to compute $\bar n$. Let $\phi$ be an arbitrary function on
$M$. We can extend $\phi$ to all of $\bar M = M \times \IR$ by setting
$\phi$ to be constant along the vertical direction. Restricting to $N$
yields a function on $N$, which we also denote by $\phi$. The
gradient of $\phi$ along $N$ satisfies
\begin{equation*}
  \nabN \phi = \nabM \phi - \la \nabM \phi, V \ra\bar\nu.
\end{equation*}
The normal $\bar n$ of $\bar S_z$ in $N$ is given by
\begin{equation*}
  \bar n
  =
  -\frac{\nabN f}{|\nabN f|}
\end{equation*}
with $\nabN f = \nabM f - \alpha^{-1}|\nabM f|^2 \bar\nu$ and $|\nabN
f|^2 = |\nabM f|^2 - \la \nabM f, V \ra^2 = \alpha^{-2}|\nabM f|^2$.
This yields that
\begin{equation*}
  \bar n
  =
  - \alpha \frac{\nabM f}{|\nabM f|} + |\nabM f|\bar \nu
  =
  \alpha n + |\nabM f|\bar \nu.
\end{equation*}
Since $\bar\nu = \alpha^{-1}(\nabla f - \del_z)$, the horizontal projection
of $\bar n$ satisfies
\begin{equation*}
  \pi\bar n = \alpha^{-1} n.
\end{equation*}
Recall that $\xi = \nabN \log v + K(\bar\nu, \cdot)^T$, whence
\begin{equation*}
  \la \xi,\bar n\ra
  =
  \nabN_{\bar n} \log v + \bar K(\bar\nu,\bar n)
  =
  \nabN_{\bar n} \log v + \frac{|\nabM f|}{\alpha^2}K(n,n).
\end{equation*}
For $v=\alpha^{-1}$ we compute that
\begin{equation*}
  \nabM \log v = \alpha^{-1}|V|\nabla^2(n, \cdot).
\end{equation*}
As before,
\begin{equation*}
  \nabN\log v = \nabM\log v - \la \nabM\log v,V\ra \bar \nu,
\end{equation*}
and thus
\begin{equation*}
  \begin{split}
    \la \nabN\log v , \bar n\ra
    &=
    \la \nabM \log v, \bar n\ra
    =
    \la \nabM \log v, \pi \bar n\ra
    \\
    &=
    \alpha^{-1} \la \nabM \log v, n\ra
    =
    \alpha^{-2}|V| \nabla^2 f(n,n).
  \end{split}
\end{equation*}
We infer that
\begin{equation*}
  \la \xi,\bar n\ra
  =
  \alpha^{-2} |V|\nabla^2f(n,n) - \alpha^{-1} |V| K(n,n).
\end{equation*}
Recall that $\nabla_n |V| = - \alpha^{-3}\nabla^2 f(n,n)$ and hence
\begin{equation*}
  \la \xi,\bar n\ra
  =
  -\alpha |V| \nabla_n |V| - \alpha^{-1}|V| K(n,n).
\end{equation*}
We compute that
\begin{equation*}
  \alpha = (1-|V|^2)^{-1/2}, 
\end{equation*}
inserting this yields
\begin{equation}
  \label{eq:9}
  \la \xi,\bar n\ra
  =
  - \frac{|V|\nabla_n|V|}{\sqrt{1-|V|^2}}
  - \sqrt{1-|V|^2}|V| K(n,n).
\end{equation}
Clearly, as $z\to\infty$ the second term goes to zero, since $|V|\to
1$, so we only have to consider the first term.

Let $\gamma_p$ be a curve starting at $p\in\del M$ such that
$\gamma_p$ is the integral curve for the vector field $n$. Define
$\phi_p(s):=|V|(\gamma_p(s))$. Then from the above considerations, we
infer that $\phi_p$ satisfies $\phi'_p(0)=0$. Differentiating
equation~\eqref{eq:14} with respect to $n$ yields
\begin{equation*}
  \begin{split}
    0
    &=
    \phi_p''(s)
    + \phi_p'(s) \theta^+
    + \phi_p(s) \nabla_n \theta^+
    - \phi_p'(s) P
    + (1-\phi_p(s)) \nabla_n P
    \\
    &\phantom{=}     
    - 2\phi_p(s) \phi_p'(s) K(n,n)
    + (1-\phi_p(s)^2) \nabla_n K(n,n)    
  \end{split}
\end{equation*}
in the limit $s\to 0$ we have $\phi_p(s)\to 1$ and $\phi_p'(s)\to
0$. Thus
\begin{equation*}
  \phi''_p(0) = - \nabla_n\theta^+.
\end{equation*}
Thus we infer the expansion 
\begin{equation}
  \label{eq:10}
  \phi_p(s) = 1 - \half \nabla_n\theta^+ s^2 + o(s^2),
\end{equation}
as $s\to 0$. Since $\phi(0)=1$ and $\phi\leq 1$ we infer that
$\nabla_n\theta^+ \geq 0$. In the case $\nabla_n\theta^+ >0$ we can
explicitly compute the limit in equation~\eqref{eq:9}:
\begin{equation*}
  \begin{split}
    \lim_{s\to 0} \la \xi,\bar n\ra(\gamma_p(s))
    &=
    -\lim_{s\to 0} \frac{\phi_p(s) \phi'_p(s)}{\sqrt{1-\phi_p(s)^2}}
    =
    -\lim_{s\to 0} \frac{\phi'_p(s)}{\sqrt{2}\sqrt{1-\phi_p(s)}}
    \\
    &=
    \lim_{s\to 0} \frac{\nabla_n\theta^+s +o(s)}
                     {\sqrt{2}\sqrt{\nabla_n\theta^+} s + o(s)}
    =
    \sqrt{\nabla_n \theta^+}.
  \end{split}
\end{equation*}
In the case $\nabla_n\theta^+ =0$ we can not explicitly compute the
limit. However, since $\phi <1$ for $s>0$, we can introduce the
function $\omega$ by setting
\begin{equation*}
  \phi(s) = \cos\omega(s)
\end{equation*}
where we choose $\omega\geq 0$. As $\phi'= -\omega'\sin\omega$ we can
write the first term in~\eqref{eq:9} as
\begin{equation*}
  \frac{\phi'(s)}{\sqrt{1-\phi'(s)^2}}
  =
  \frac{-\omega'(s)\sin\omega}{\sin\omega}
  =
  -\omega'(s)
\end{equation*}
as $\phi<1$ we find that $\omega'(0)\geq 0$ and thus
\begin{equation*}
  \liminf_{s\to 0} \la \xi,\bar n \ra (\gamma_p) \geq 0.
\end{equation*}
Hence, we arrive at the main result of this section
\begin{theorem}
  Let $(M,g,K)$ be a data set as in theorem~\ref{thm:blowup} with the
  extra condition that $\del M$ be strictly stable. Let $f$ be the
  solution to Jang's equation constructed there. Let $S_z=\{ f= z\}$
  be the level set of $f$ for large enough $z\geq \bar z$, let $\bar
  n$ be the normal vector to $\graph f \cap M\times\{z\}$ in $\graph
  f$ and let $\xi$ be defined as in equation~\eqref{eq:11}. Then
  \begin{equation*}
    \liminf_{s\to 0} \la\xi, \bar n\ra(\gamma(s)) \geq 0
  \end{equation*}
  for all curves $\gamma$ starting on $\del M$ with tangent
  $\dot\gamma(0)$ transversal to $\del M$.
\end{theorem}
If $(M,g,K)$ is radially symmetric, $\nabla_n \theta^+$ is constant
along $\del M$ and equals the smallest eigenvalue $\lambda$ of the
$\theta^+$-stability operator of $\del M$. In this case we find an
example where $\la\xi,\bar\nu\ra$ is strictly positive on $\del M$.
\begin{corollary}
  If $(M,g,K)$ is as in theorem~\ref{thm:blowup} and additionally
  rotationally symmetric, including $\del M$, then if $\del M$ is a
  strictly stable MOTS, we have
  \begin{equation*}
    \lim_{s\to 0} \la\xi,\bar\nu\ra(s) = \sqrt{\lambda}>0
  \end{equation*}
  where $s$ denotes the radial distance to $\del M$.
\end{corollary}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 


==> draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}
\newcommand{\thmfamily}{}
\newcommand{\sectitlefnt}{}
\newcommand{\subsectitlefnt}{}
\newcommand{\ps@footnumber}{}

\newcommand{\authname}[1]{#1}
\newcommand{\authaddress}[1]{#1}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=136mm,totalheight=213mm,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}

  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }

  \renewcommand{\authname}[1]{\titlefamily #1\hspace*{0pt}\\}
  \renewcommand{\authaddress}[1]{\begin{minipage}{.8\linewidth}\centering\titlefamily\footnotesize
      #1\hspace*{0pt}\end{minipage}\\[1ex]}
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

